Designing Short-Stage CDC-XPUFs: Balancing Reliability, Cost, and Security in IoT Devices

The rapid expansion of Internet of Things (IoT) devices demands robust and resource-efficient security solutions. Physically Unclonable Functions (PUFs), which generate unique cryptographic keys from inherent hardware variations, offer a promising approach. However, traditional PUFs like Arbiter PUFs (APUFs) and XOR Arbiter PUFs (XOR-PUFs) are susceptible to machine learning (ML) and reliability-based attacks. In this study, we investigate Component-Differentially Challenged XOR-PUFs (CDC-XPUFs), a less explored variant, to address these vulnerabilities. We propose an optimized CDC-XPUF design that incorporates a pre-selection strategy to enhance reliability and introduces a novel lightweight architecture to reduce hardware overhead. Rigorous testing demonstrates that our design significantly lowers resource consumption, maintains strong resistance to ML attacks, and improves reliability, effectively mitigating reliability-based attacks. These results highlight the potential of CDC-XPUFs as a secure and efficient candidate for widespread deployment in resource-constrained IoT systems.

==> sec3_unused.tex <==
\section{Delay Difference and PUF Reliability}

The robustness and reliability of PUFs are critical for their application in security systems. This section discusses the fundamental concepts of delay differences in APUFs, which are central to their functionality and directly impact their vulnerability to noise and reliability performance. By understanding these core dynamics, we can better appreciate the need for and the implementation of strategies that enhance PUF reliability, such as the pre-selection strategy discussed later.

\subsection{Fundamental Concepts of Delay Difference}


In Arbiter PUFs (APUFs), the core determinant of the binary response is the delay difference $(\Delta D)$ between two competing signal paths. These paths are modulated by the binary `challenge' applied to the PUF. The delay difference $\Delta D$ is defined as the difference between the delay encountered by the signal on the upper path $(d_{\text{upper}})$ and the lower path $(d_{\text{lower}})$, formally expressed as:
\begin{equation}
\Delta D = d_{\text{upper}} - d_{\text{lower}}
\end{equation}

\subsection{Impact of Noise on PUF Responses}


The binary response $(r)$ of the PUF is determined by the sign of $\Delta D$. In the absence of electronic noise and other perturbations, the response is given by:
\begin{equation}
r = \text{Sign}(\Delta D)
\end{equation}
Where:
\begin{itemize}
    \item $r = 1$ if $\Delta D < 0$ (i.e., the signal on the lower path is faster).
    \item $r = 0$ otherwise (i.e., the signal on the upper path is faster).
\end{itemize}

\textbf{Incorporation of Noise:}
In practical scenarios, electronic noise and environmental variations introduce a noise term $(d_{\text{noise}})$, which affects the delay measurements. The response with noise can then be modeled as:
\begin{equation}
r = \text{Sign}(\Delta D \pm d_{\text{noise}})
\end{equation}
Where $d_{\text{noise}}$ represents the variability introduced by noise, and the `$\pm$' sign indicates that noise can either increase or decrease the measured delay difference.


A critical observation is that the reliability of the PUF response is contingent upon the magnitude of $\Delta D$. If $\Delta D$ is large, it is highly unlikely that the noise term $d_{\text{noise}}$ will be sufficient to change the sign of $\Delta D$, thereby preserving the integrity of the response. Conversely, when $\Delta D$ is small, even minimal noise can result in erroneous responses, making such CRPs unreliable.

\subsection{Pre-selection strategy to improve reliability}

Based on the observation of noise impact the reliability of PUF responses is significantly influenced by the magnitude of $\Delta D$, large values of $\Delta D$ ensure that the noise term $d_{\text{noise}}$ is unlikely to alter the outcome of $\text{Sign}(\Delta D)$, leading to stable and reliable responses. This critical observation motivates the implementation of a pre-selection strategy wherein CRPs are evaluated and selected based on the robustness of their delay differences. Only those CRPs where $\left|\Delta D\right|$ exceeds a predefined threshold are utilized, significantly enhancing the PUF's reliability by mitigating noise-induced response fluctuations.

To operationalize the pre-selection strategy, we introduce additional delay elements into the traditional PUF architecture to selectively manipulate the delay paths based on the observed $\Delta D$ values. The following figure \ref{fig:apuf_preselection} illustrates this implementation:

\begin{figure*}[htbp]
    \centering
    \includegraphics[width=0.8\textwidth]{delay.png}
    \caption{Implementation of the pre-selection strategy in an Arbiter PUF, illustrating the conditional path adjustments for enhancing response reliability.}
    \label{fig:apuf_preselection}
\end{figure*}


To enhance the reliability of responses, we implement a pre-selection strategy that involves evaluating three potential responses for each challenge:
\begin{itemize}
    \item \textbf{Response1:} $\text{Sign}(d_{\text{upper}} - d_{\text{lower}})$
    \item \textbf{Response2:} $\text{Sign}(d_{\text{upper}} + D_{\text{Delay module}} - d_{\text{lower}})$
    \item \textbf{Response3:} $\text{Sign}(d_{\text{upper}} - (d_{\text{lower}} + D_{\text{Delay module}})$
\end{itemize}

CRPs are selected for use only if all three responses are consistent, i.e., all are "000" or "111". This condition ensures that the absolute difference $|d_{\text{upper}} - d_{\text{lower}}|$ is greater than the "Delay module", indicating a robust delay difference that is likely to be resilient to noise impacts. This setup ensures that only the CRPs with significant delay differences, and thus higher reliability, are selected for security applications. 






==> sec4_unused.tex <==


\section{Pre-selection Strategy Experimental Validation}

Experiments were conducted using two types of FPGA boards: Artix-7 A7-35T and NEXYS A7-50T. Each board type included three distinct units, with five PUF instances each, thereby creating a robust dataset for comprehensive analysis across different hardware implementations.

\subsection{Experimental Setup}

\textbf{CRP Generation:}
A total of 100 million CRPs were generated for each PUF instance utilizing a pseudorandom number generator (PRNG). The PRNG was defined by the equation:
\begin{equation}
    C_{n+1} = (a \times C_n + g) \mod m,
\end{equation}
where $C$ represents the sequence of generated numbers, $a$ is a multiplier, $g$ is a constant adder, and $m$ is $2^K$, with $K$ being the number of stages. CRPs were selectively filtered to include only those producing uniform "000" or "111" responses, ensuring significant delay differences $(\Delta D)$ and enhanced reliability.

\textbf{Delay Modules Configuration:}
Two configurations were tested to explore their impact on PUF performance: 
1. Modules with two or four NOT gates.
2. Modules with one, two, or three AND gates.

These configurations introduced controlled delays in the signal paths, allowing the examination of their effects on PUF performance under varied conditions.

\textbf{Tool Configuration and Data Handling:}
The PUF architectures were designed using VHDL within the Xilinx Vivado 15.4 HL Design Edition software suite, and implemented on FPGAs using Tool Command Language (TCL) scripts for precise placement. Communication between the FPGA and the test environment was managed via the Xilinx Software Development Kit (SDK), using AXI GPIO interfaces for challenge submissions and response collections, and AXI UART for data transmission at a rate of 230,400 bits per second, facilitated by Tera Term.

\textbf{Reliability Testing:}
To assess stability and performance, reliability tests were conducted 10,000 times per PUF instance, maintaining the operating voltage at 2.0W and ambient temperature around the Xilinx Artix\textregistered-7 FPGA at 26.0$^\circ$C, with a thermal margin of 59.0$^\circ$C (12.3W).

\subsection{Evaluation Metrics for PUF Performance}

\textbf{Uniqueness:}
Introduced by Hori et al. \cite{hori2010quantitative}, uniqueness measures the ability of PUFs to produce distinct responses across devices for the same challenges. It is quantified as:
\begin{equation}
    HU_k = \frac{4}{N_r \times N^2 }\sum_{i=1}^{N_r}\sum_{j,m=1, j\ne m}^{N} (b_{j,i} \oplus b_{m,i}),
\end{equation}
where $N$ is the number of chips, $N_r$ is the response length, and $b_{j,i}$, $b_{m,i}$ are the $i$-th response bits from the $j$-th and $m$-th PUF instances, respectively.

\textbf{Reliability (BER):}
The Bit Error Rate (BER) quantifies the consistency of PUF outputs under identical conditions and is defined as:
\begin{equation}
    \text{BER} = 1 - R = \frac{N - \sum_{i=1}^{N} (b_i == b_{ref})}{N},
\end{equation}
where a lower BER indicates higher reliability.

\textbf{Randomness:}
Randomness evaluates the balance of '0's and '1's in PUF responses to ensure unpredictability:
\begin{equation}
    p = \frac{1}{N_r} \sum_{i=1}^{N_r} b_i,
\end{equation}
\begin{equation}
    H = -\log_{2}\max(p, 1 - p),
\end{equation}
where $N_r$ is the total number of responses, and $b_i$ is a response bit.

\subsection{Experimental Results}

The results, summarized in Table \ref{fig:experimental_result1}, indicate that the pre-selection strategy significantly enhances reliability, showing a substantial reduction in BER and maintaining high uniqueness and randomness. 

Step further, configurations utilizing two delay gates emerged as particularly effective, achieving an optimal balance between securing reliability and maintaining an acceptable selection rate. Specifically, two delay gates ensured enhanced reliability of the PUF responses, with approximately 5\% of CRPs being reliably filtered. This rate is considered acceptable given that the PUFs tested are capable of providing an exponentially large CRP space, ensuring a sufficient number of CRPs remain usable for robust authentication and security applications.

Conversely, while one delay gate did increase reliability compared to no delay modification, the improvements were not substantial enough to deem this configuration reliable under all expected operational conditions. Thus, one delay gate falls short of providing the desired level of dependability needed for critical applications.

The configuration with four delay gates, although potentially offering the highest level of reliability, resulted in an overly restrictive selection rate of merely 0.06\% to 0.2\% of CRPs. Such a low rate severely limits the practical usability of the PUF, as it drastically reduces the number of available CRPs to a point that may not support diverse operational requirements, especially in scenarios demanding high-frequency authentication. 

\begin{table*}[htbp]
        \centering
        \caption{Comparison of PUF performance metrics before and after applying the pre-selection strategy, featuring different delay module configurations.}
        \linespread{1.3}\selectfont
        \setlength\tabcolsep{5pt}
        \label{fig:experimental_result1}
    \begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\textbf{PUF type} &
  \textbf{CRP generated} &
  \textbf{Implemented Delay Module} &
  \textbf{\% of selected CRP} &
  \textbf{\begin{tabular}[c]{@{}c@{}}BER\\ (ideal value 0)\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Uniqueness\\ (ideal value 1)\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Randomness\\ (ideal value 0.5)\end{tabular}} \\ \hline
\multirow{6}{*}{\textbf{APUF 64-bit}} & \multirow{14}{*}{\textbf{100m}} & \textbf{None}        & 100\%  & 0.67\%           & 42\% & 52\% \\ \cline{3-7} 
                                      &                                 & \textbf{1 AND gates} & 70\%   & 0.02\%           & 50\% & 55\% \\ \cline{3-7} 
                                      &                                 & \textbf{2 AND gates} & 6.2\%  & \textless{}10e-8 & 52\% & 58\% \\ \cline{3-7} 
                                      &                                 & \textbf{2 NOT gates} & 5.90\% & \textless{}10e-8 & 65\% & 56\% \\ \cline{3-7} 
                                      &                                 & \textbf{3 AND gates} & 0.06\% & \textless{}10e-8 & -    & -    \\ \cline{3-7} 
                                      &                                 & \textbf{4 NOT gates} & 0.02\% & \textless{}10e-8 & -    & -    \\ \cline{1-1} \cline{3-7} 
\multirow{2}{*}{\textbf{2 XOR-PUF}}   &                                 & \textbf{1 AND gates} & 51\%   & 0.02\%           & -    & -    \\ \cline{3-7} 
                                      &                                 & \textbf{2 NOT gates} & 0.5\%  & \textless{}10e-8 & -    & -    \\ \cline{1-1} \cline{3-7} 
\multirow{2}{*}{\textbf{3 XOR-PUF}}   &                                 & \textbf{1 AND gates} & 32\%   & 0.01\%           & -    & -    \\ \cline{3-7} 
                                      &                                 & \textbf{2 NOT gates} & 0.02\% & \textless{}10e-8 & -    & -    \\ \cline{1-1} \cline{3-7} 
\multirow{2}{*}{\textbf{6 XOR-PUF}}   &                                 & \textbf{1 AND gates} & 2\%   & 0.008\%           & -    & -    \\ \cline{3-7} 
                                      &                                 & \textbf{2 NOT gates} & 0\% & - & -    & -    \\ \cline{1-1} \cline{3-7} 
\multirow{2}{*}{\textbf{CDC-2-XPUF}}  &                                 & \textbf{1 AND gates} & 65\%   & 0.03\%           & 58\% & 54\% \\ \cline{3-7} 
                                      &                                 & \textbf{2 NOT gates} & 4.5\%  & \textless{}10e-8 & 60\% & 55\% \\ \cline{1-1} \cline{3-7} 
\multirow{2}{*}{\textbf{CDC-3-XPUF}}  &                                 & \textbf{1 AND gates} & 60\%   & 0.05\%           & 60\% & 52\% \\ \cline{3-7} 
                                      &                                 & \textbf{2 NOT gates} & 5.2\%  & \textless{}10e-8 & 66\% & 54\% \\ \hline
\end{tabular}
    \end{table*}

\subsection{Discussion on Applicability to XOR-PUFs}

The pre-selection strategy is effective for APUFs, however, APUFs were proven to be weak against ML modeling attacks. The reliability filtering achieved through this strategy is significantly compromised in traditional XOR-PUFs due to their composite nature, which combines outputs from multiple Arbiter PUF components. In XOR-PUFs, the variance in component reliability makes it difficult to apply a uniform pre-selection strategy effectively; a CRP that is reliable for one component may not be reliable for another, reducing the overall utility of the strategy.

These limitations are notably absent in CDC-XPUFs, which are designed to accommodate differential challenges across components. This unique architecture allows for the independent application of the pre-selection strategy to each component, significantly enhancing the overall reliability of the system. 

Experimental validation was conducted to assess the viability of applying the pre-selection strategy to both XOR-PUFs and CDC-XPUFs. The approach involved deploying arbiter PUF components with a delay module configuration on FPGA boards. The pre-selection strategy was then utilized to filter and compile a CRP sub-dataset for each component. For XOR-PUFs, a unified dataset was created by selecting challenges common across all components, whereas for CDC-XPUFs, these sub-datasets were combined to form a comprehensive dataset.

The experimental results, detailed in Table \ref{fig:experimental_result1}, illustrate the differing impacts of the pre-selection strategy on traditional XOR-PUFs and CDC-XPUFs. While the strategy enhances the reliability of individual components within CDC-XPUFs, its application in XOR-PUFs did not yield comparably beneficial outcomes. The percentage of selected reliable CRPs for XOR-PUFs remained low, underscoring the strategy's ineffectiveness in this context due to inter-component reliability variance.

Conclusively, the pre-selection strategy's success in CDC-XPUFs versus its limited efficacy in XOR-PUFs underscores the importance of component independence in PUF designs. CDC-XPUFs, with their ability to independently handle differential challenges, offer a more robust and flexible framework for implementing reliability-enhancing strategies such as pre-selection. 

